Neural Packing: from Visual Sensing to Reinforcement Learning

We present a novel learning framework to solve the transport-and-packing (TAP) problem in 3D. It constitutes a full solution pipeline from partial observations of input objects via RGBD sensing and recognition to final box placement, via robotic motion planning, to arrive at a compact packing in a target container. The technical core of our method is a neural network for TAP, trained via reinforcement learning (RL), to solve the NP-hard combinatorial optimization problem. Our network simultaneously selects an object to pack and determines the final packing location, based on a judicious encoding of the continuously evolving states of partially observed source objects and available spaces in the target container, using separate encoders both enabled with attention mechanisms. The encoded feature vectors are employed to compute the matching scores and feasibility masks of different pairings of box selection and available space configuration for packing strategy optimization. Extensive experiments, including ablation studies and physical packing execution by a real robot (Universal Robot UR5e), are conducted to evaluate our method in terms of its design choices, scalability, generalizability, and comparisons to baselines, including the most recent RL-based TAP solution. We also contribute the first benchmark for TAP which covers a variety of input settings and difficulty levels.

==> figures/approximate_test.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.49\textwidth]{images/approximate_test.pdf}
\caption{\rh{Packing results of networks training on with different quantization levels when tested on the same set of shapes but with size approximated using the corresponding quantization level.}}
\label{fig:approximate_test}
\end{figure}


==> figures/baseline_example.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.98\textwidth]{images/baseline_example_compressed.pdf}
\caption{Comparison of packing results between our method and two baseline methods under practical settings. In the last test, our approach uses only two containers, whereas the other two approaches use three. \jzc{need to update}}
\label{fig:baseline_example}
\end{figure*}


==> figures/baseline_example2.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.98\textwidth]{images/baseline_example2_compressed.pdf}
\caption{Comparison of packing results between TAP-Net++ and two baseline methods under constrained settings. Note that in the first case, Greedy EMS uses two containers, whereas TAP-Net and TAP-Net++ pack all objects into one. \jzc{need to update}} 
	%\mlc{I suggest putting the first (fully) packed container on the left side.}
\label{fig:baseline_example2}
\end{figure*}


==> figures/diff_prec.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.49\textwidth]{images/diff_prec.pdf}
\caption{Under different quantization levels, the same real object is approximated by boxes of different sizes (shown as transparent boxes). As the unit length increases, the approximation becomes more coarse.}
\label{fig:diff_prec}
\end{figure}


==> figures/object_detection.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.49\textwidth]{images/object_detection.pdf}
\caption{Object extraction. Given the RGBD image captured from the source objects, our method first uses the Mask RCNN network~\cite{he2017mask} to detect the objects, and then uses the cuboid fitting algorithm~\cite{jiang2013linear} to estimate the size and 6D pose of each detected object.}
\label{fig:detect}
\end{figure}


==> figures/real_env.tex <==
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{images/real_env.jpg}
	\caption{\change{A photograph taken of a real-world working environment at a robotics company. All the boxes stacked up on one side of the space must be packed into target containers. At present, a human operator has to manually pick up and place the boxes onto the conveyor belt, one by one, for the robotic arm to transport them into the containers. This practice is not only tedious for the operator but also potentially unsafe, whether due to the weight of the boxed products or operating close to heavy machinery. An automated solution allowing the robotic arm to directly transport-and-pack the boxes from their stacked state to the target containers would be highly desirable, as confirmed by the company personnel.}}
	\label{fig:real_env}
\end{figure}


==> figures/real_robot.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.99\textwidth]{images/real_robot.pdf}
\caption{\rh{Packing for real.}}
\label{fig:real_robot}
\end{figure*}


==> figures/rotation_3D.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.49\textwidth]{images/3D_rotation_reduced.pdf}
\caption{Six different object rotation states in 3D (bottom 2 rows) and the corresponding robot arm access approach (top row). The first two states (left column) only require the top of the box being accessible, whereas the remaining four also require one of the sides being accessible.}
\label{fig:rotation_3D}
\end{figure}


==> figures/shape_encoder.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.49\textwidth]{images/shape_encoder.pdf}
\caption{The detailed structure of the object encoder as part of the Source Encoder in Figure~\ref{fig:network}.}
\label{fig:shape_enc}
\end{figure}


==> figures/tab_ablation.tex <==
\begin{table}[!t]%
	\caption{Ablation studies of TAP-Net++ on precedence encoder used for source boxes (left) and packing corner selection for box and EMS alignment (right).}
	\label{tab:ablation}
	\begin{minipage}{\columnwidth}
		\begin{center}

		\begin{tabular}{ l l l || l l}
			
			\hline
			
			 \multicolumn{3}{l||}{\textbf{Precedence encoder}} & \multicolumn{2}{l}{\textbf{ Packing corners}} \\  \hline
			
			  \multicolumn{1}{l|}{CNN} & \multicolumn{1}{l|}{RNN} & \multicolumn{1}{l||}{\textbf{\small Transformer}} &  \multicolumn{1}{l|}{All four corners} & \multicolumn{1}{l}{\textbf{\small DBL corner}}  \\ \hline
			
			  \multicolumn{1}{l|}{0.813} & \multicolumn{1}{l|}{0.806} & \multicolumn{1}{l||}{\textbf{0.818}} &  \multicolumn{1}{l|}{0.813} & \multicolumn{1}{l}{\textbf{0.818}} \\ \hline
			
		\end{tabular}
	
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_ablation_attention.tex <==
\begin{table}[!t]%
	\caption{Comparison on network performance when using attention module vs a transformer-based encoder for feature extraction.}
	\label{tab:ablation_attn}
	\begin{minipage}{\columnwidth}
		\begin{center}
		\begin{tabular}{l||l}
			\hline
			\textbf{Encoder} &  \bm{$C$}  \\ \hline
			Transformer & 0.815 \\ \hline
			\textbf{Attention} & \textbf{0.818} \\ \hline
		\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_ablation_ems.tex <==
\begin{table}[!t]%
	\caption{Performance of TAP-Net++ when different strategies are used for computing packing locations.}
	\label{tab:ablation_ems}
	\begin{minipage}{\columnwidth}
		\begin{center}
		\begin{tabular}{l||l}
			\hline
			\textbf{Corner} &  \bm{$C$}  \\ \hline 
			align the DBL corner only & \textbf{0.818} \\ \hline
			try all 4 corners at bottom & 0.813 \\ \hline
		\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_ablation_precd.tex <==
\begin{table}[!t]%
	\caption{Performance of TAP-Net++ with different precedence encoders.}
	\label{tab:ablation_precd}
	\begin{minipage}{\columnwidth}
		\begin{center}
		\begin{tabular}{l||l}
			\hline
			\textbf{Encoder} &  \bm{$C$} \\ \hline
			CNN & 0.813 \\ \hline
			RNN & 0.806 \\ \hline
			\textbf{Transformer} & \textbf{0.818} \\ \hline
		\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_approximate_test.tex <==
\begin{table}[!t]%
	\caption{Performance (Compactness) of TAP-Net++ trained and tested under different quantization levels (unit lengths $u$).
	Note that the actual object dimensions are used for compactness evaluation, even though their approximate dimensions are fed to TAP-Net++ for training and testing.
	}
	\label{tab:approximate_test}
	\begin{minipage}{\columnwidth}
		\begin{center}
		
		\begin{tabular}{l||l|l|l|l}
			\hline
			\diagbox{Trained $u$}{Tested $u$} &  20 & 10 & 5 & 1 \\ \hline
			20 & 0.522 & 0.577	 & 0.610 & 0.638 \\ \hline
			10 & -    & 0.588 	& 0.619 & 0.648 \\ \hline
			5 & -     & -    	& 0.623 & 0.647 \\ \hline
			1 & -     & - 		& - 	& 0.648 \\ \hline
		\end{tabular}

	
		\end{center}
	\end{minipage}
\end{table}%



%\textbf{Training precision} & \multicolumn{1}{l|}{\textbf{Approximate $\rightarrow$ Actual}} & \textbf{Actual} \\ \hline \hline 
%20 & \multicolumn{1}{l|}{0.777 $\rightarrow$ 0.470} & 0.638 \\ \hline
%10 & \multicolumn{1}{l|}{0.725 $\rightarrow$ 0.557} & 0.648 \\ \hline
%5 & \multicolumn{1}{l|}{0.683 $\rightarrow$ 0.606} & 0.647 \\ \hline
%1 & \multicolumn{2}{l}{0.648} \\ \hline \hline 


==> figures/tab_baseline.tex <==
\begin{table}[!t]%
	\caption{Comparison on the performance of the full pipeline obtained using TAP-Net++ and the two baseline methods.}
	\label{tab:baseline}
	\begin{minipage}{\columnwidth}
		\begin{center}
		\begin{tabular}{l||l|l}
			\hline
			\textbf{Method} &  \bm{$C$} & \bm{$N_{\text{ctn}}$}  \\ \hline 
			Greedy EMS & 0.638 & 2.398 \\ \hline
			% Greedy PCT &   &   \\ \hline
			TAP-Net & 0.619 & 2.582 \\ \hline
			\textbf{TAP-Net++} & \textbf{0.692} & \textbf{2.294} \\ \hline
		\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_box_num.tex <==
\begin{table}[!t]%
	\caption{\jz{Scalability on box num.}}
	\label{tab:tab_scalability_num}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l||l | l | l }
				\hline
				
				\textbf{\bm{{$N_{box}$}}} &  \bm{$C$} & \bm{$N$} & \bm{$\Delta N$}   \\ \hline 
				20 &   &    &    \\ \hline
				40 &   &    &    \\ \hline
				60 &   &    &    \\ \hline
				80 &   &    &    \\ \hline
				100 &   &    &    \\ \hline
				
				
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_diff_num_height_limit.tex <==
\begin{table}[!t]%
	\caption{\jz{Performance of TAP-Net++ trained and tested different box numbers $N_{\text{obj}}$.  
	TAP-Net++ trained on fewer boxes generalizes well for more boxes.}}
		%\ml{Performance of TAP-Net++ on tasks with 20 boxes but trained on datasets with different box numbers $N_{obj}$. The TAP-Net++ trained on fewer boxes generalizes well for more boxes.} 
		%\mlc{I felt that we do not need to test different unit length here.  if there is time, it is helpful to test another box numbers (50) and test how well network trained using more boxes perform on fewer boxes (a matrix of performance between input and output box number.)} }
	\label{tab:diff_num_height_limit}
	\begin{minipage}{\columnwidth}
		\begin{center}	
		
		\begin{tabular}{l || l l l  l l l}
			
			\hline
			
			\textbf{Trained $N_{obj}$} & \multicolumn{3}{l|}{10} & \multicolumn{3}{l}{20} \\ \hline
			
			\textbf{Tested $N_{obj}$} &  \multicolumn{1}{l|}{10} & \multicolumn{1}{l|}{20} & \multicolumn{1}{l|}{50} &  \multicolumn{1}{l|}{10} & \multicolumn{1}{l|}{20} & \multicolumn{1}{l}{50} \\ \hline
			
			\textbf{TAP-Net} &  \multicolumn{1}{l|}{0.672} & \multicolumn{1}{l|}{0.675} & \multicolumn{1}{l|}{0.667} &  \multicolumn{1}{l|}{0.620} & \multicolumn{1}{l|}{0.634} & \multicolumn{1}{l}{0.626} \\ \hline
			
			\textbf{TAP-Net++} &  \multicolumn{1}{l|}{\textbf{0.757}} & \multicolumn{1}{l|}{\textbf{0.776}} & \multicolumn{1}{l|}{\textbf{0.782}} &  \multicolumn{1}{l|}{\textbf{0.708}} & \multicolumn{1}{l|}{\textbf{0.753}} & \multicolumn{1}{l}{\textbf{0.772}} \\ \hline
			
		\end{tabular}
		
	
	
		\end{center}
	\end{minipage}
\end{table}%


%\begin{tabular}{l || l l l l  l l  l l }
	
%	\hline
%	\bm{$u$} &  \multicolumn{2}{l|}{20} & \multicolumn{2}{l|}{10} & \multicolumn{2}{l|}{5} & \multicolumn{2}{l}{1}  \\ \hline
	
%	\bm{$N_{obj}$} & \multicolumn{1}{l|}{10} & \multicolumn{1}{l|}{20} & \multicolumn{1}{l|}{10} & \multicolumn{1}{l|}{20} & \multicolumn{1}{l|}{10} & \multicolumn{1}{l|}{20} & \multicolumn{1}{l|}{10} & \multicolumn{1}{l}{20} \\ \hline
	
%	\textbf{TAP-Net} & \multicolumn{1}{l|}{0.769} & \multicolumn{1}{l|}{0.772} & \multicolumn{1}{l|}{0.671} & \multicolumn{1}{l|}{0.681} & \multicolumn{1}{l|}{0.573} & \multicolumn{1}{l|}{0.610} & \multicolumn{1}{l|}{0.557} & \multicolumn{1}{l}{0.526}  \\ \hline
	
%	\textbf{TAP-Net++} & \multicolumn{1}{l|}{\textbf{0.834}} & \multicolumn{1}{l|}{\textbf{0.859}} & \multicolumn{1}{l|}{\textbf{0.744}} & \multicolumn{1}{l|}{\textbf{0.758}} & \multicolumn{1}{l|}{\textbf{0.697}} & \multicolumn{1}{l|}{\textbf{0.709}} & \multicolumn{1}{l|}{\textbf{0.635}} & \multicolumn{1}{l}{\textbf{0.679}} \\ \hline
	
%\end{tabular}

==> figures/tab_diff_prec.tex <==
\begin{table}[!t]%
	\caption{Performance of TAP-Net++ trained on data with different quantization levels, but all tested on data with unit length $u=1$.
	For each test shape, we represent it using either the \emph{approximate} size with the training quantization level $u$ or the \emph{actual} size with $u=1$ to get two sets of results. 
	\mlc{it is a bit confusing here to explain approximate vs actual.  Can we test a matrix of performance between Du and Tu? Du=20 vs Tu=20, 10, 5, 1;  Du=20 vs Tu=10, 5, 1; Du=5 vs Tu=5, 1.}}
	\label{tab:diff_prec}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l||l|l|l|l}
				\hline
				\textbf{Training $u$} & 20 & 10 & 5 & 1 \\ \hline
				\textbf{Approximate} & 0.522 & 0.588 & 0.623 & 0.648 \\ \hline
				\textbf{Actual} & 0.638 & 0.648 & 0.647 & 0.648 \\ \hline
			\end{tabular}
			
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_eval_prec.tex <==
\begin{table}[!t]%
	\caption{Performance comparison between our network and baseline methods under different container sizes. Each task contains 10 source objects, which are axis-aligned and with known configurations, as in TAP-Net~\cite{hu2020tap}. The average Compactness ($C$) for 1,000 tasks are reported.} 
	%All experiments are tested on tasks with 10 boxes.}
	\label{tab:eval_prec}
	\begin{minipage}{\columnwidth}
		\begin{center}
			
		\begin{tabular}{l||l|l|l|l}
			\hline
			\textbf{Container size} &  \textbf{5} & \textbf{10} & \textbf{20} & \textbf{100} \\ \hline
			Greedy EMS & 0.703 & 0.643 & 0.587 & 0.583 \\ \hline
			% Greedy PCT &   &   &  &  \\ \hline
			TAP-Net & 0.747 & 0.652 & 0.591 & 0.536 \\ \hline
			\textbf{TAP-Net++} & \textbf{0.818} & \textbf{0.718} & \textbf{0.666} & \textbf{0.648} \\ \hline
		\end{tabular}
		
		%\begin{tabular}{l||l|ll}
		%	\hline\hline
		%	\multicolumn{1}{c||}{\multirow{2}{*}{Method}} & Infinity height & \multicolumn{2}{c}{Finity height} \\ \cline{2-4}
		%	\multicolumn{1}{c||}{}   & C & \multicolumn{1}{l|}{C} & N \\ \hline \hline
		%	Greedy DBLF & 1 & \multicolumn{1}{l|}{1} & 1 \\ \cline{1-4}
		%	TAP-Net & 1 & \multicolumn{1}{l|}{1} & 1  \\ \cline{1-4}
		%	\textbf{TAP-Net++} & 1 & \multicolumn{1}{l|}{1} & 1 \\ \hline \hline		
		%\end{tabular}
		
		
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_fix_real_multi.tex <==
\begin{table}[!t]%
	\caption{\jz{Comparison on the performance of the full pipeline obtained using TAP-Net++ and the two baseline methods. Try to pack the FIX boxes into multiple containers}}
	\label{tab:fix_real_multi}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l||l|l|l|l}
				\hline
				\textbf{Container setting} &  \textbf{Method} & \bm{$C$} & \bm{$N$} & \bm{$\Delta N$}   \\ \hline 
				\multirow{3}{*}{Pack in last container} & Greedy & 0.361 & 5.20 &  2.91 \\ \cline{2-5}
				& TAP-Net & 0.374 & 4.99 & 2.70  \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.491} & \textbf{3.78} & \textbf{1.49} \\ \hline
				
				\multirow{3}{*}{Pack in all containers} & Greedy & 0.430 & 4.34 & 2.05 \\ \cline{2-5}
				& TAP-Net & 0.436 & 4.38 & 2.08  \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.501} & \textbf{3.78} & \textbf{1.49} \\ \hline
				
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_fix_single.tex <==
\begin{table}[!t]%
	\caption{\jz{Comparison on the performance of the full pipeline obtained using TAP-Net++ and the two baseline methods. Try to pack the FIX boxes into one container.}}
	\label{tab:fix_single}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l||l|l|l}
				\hline
				\textbf{Method} & Greedy & TAP-Net & TAP-Net++  \\ \hline 
				 \bm{$C$} & 0.614 & 0.379 & \textbf{0.657} \\ \hline
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_ppsg_ideal_multi_all.tex <==
\begin{table}[!t]%
	\caption{\jz{Comparison on the performance of the full pipeline obtained using TAP-Net++ and the two baseline methods. Testing under ideal scene, ask to pack all the PPSG boxes into multiple containers, the box can be packed in each container.}}
	\label{tab:ppsg_ideal_multi_all}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l||l|l|l|l}
				\hline
				\textbf{Unit length} &  \textbf{Method} & \bm{$C$} & \bm{$N$} & \bm{$\Delta N$}  \\ \hline 
				\multirow{3}{*}{10} & Greedy EMS & 0.633 & 1.74 & 0.73 \\ \cline{2-5}
				& TAP-Net & 0.498 & 2.02 & 1.01 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.803} & \textbf{1.40} & \textbf{0.40} \\ \hline
				\multirow{3}{*}{5} & Greedy EMS & 0.623 & 1.75 & 0.76 \\ \cline{2-5}
				& TAP-Net & 0.485 & 2.09 & 1.09 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.788} & \textbf{1.43} & \textbf{0.42} \\ \hline
				\multirow{3}{*}{1} & Greedy EMS & 0.594 & 1.81 & 0.81 \\ \cline{2-5}
				& TAP-Net & 0.486 & 2.08 & 1.08 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.783} & \textbf{1.44} & \textbf{0.43} \\ \hline	
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_ppsg_ideal_multi_last.tex <==
\begin{table}[!t]%
	\caption{\jz{Comparison on the performance of the full pipeline obtained using TAP-Net++ and the two baseline methods. Testing under ideal scene, ask to pack all the PPSG boxes into multiple containers, the box is only allowed to be packed in the last container.}}
	\label{tab:ppsg_ideal_multi_last}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l||l|l|l|l}
				\hline
				\textbf{Unit length} &  \textbf{Method} & \bm{$C$} & \bm{$N$} & \bm{$\Delta N$}  \\ \hline 
				\multirow{3}{*}{10} & Greedy EMS & 0.623 & 1.75 & 0.76 \\ \cline{2-5}
				& TAP-Net & 0.496 & 2.02 & 1.02 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.803} & \textbf{1.40} & \textbf{0.40} \\ \hline
				\multirow{3}{*}{5} & Greedy EMS & 0.621 & 1.76 & 0.76 \\ \cline{2-5}
				& TAP-Net & 0.495 & 2.04 & 1.04 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.753} & \textbf{1.50} & \textbf{0.49} \\ \hline
				\multirow{3}{*}{1} & Greedy EMS & 0.593 & 1.82 & 0.82 \\ \cline{2-5}
				& TAP-Net & 0.489 & 2.06 & 1.06 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.745} & \textbf{1.51} & \textbf{0.51} \\ \hline	
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_ppsg_ideal_single.tex <==
\begin{table}[!t]%
	\caption{\jz{Comparison on the performance of the full pipeline obtained using TAP-Net++ and the two baseline methods. Testing under an ideal scene, try to pack the PPSG boxes into one container.}}
	\label{tab:ppsg_ideal_single}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l||l|l|l}
				\hline
				\textbf{Unit length} &  \textbf{Method} & \bm{$C$} & \bm{$N_{\text{box}}$}  \\ \hline 
				\multirow{3}{*}{10} & Greedy EMS & 0.862 & 8.76 \\ \cline{2-4}
				& TAP-Net & 0.648 & 6.03 \\ \cline{2-4}
				& \textbf{TAP-Net++} & \textbf{0.947} & \textbf{9.21} \\ \hline
				\multirow{3}{*}{5} & Greedy EMS & 0.842 & 8.53 \\ \cline{2-4}
				& TAP-Net & 0.602 & 3.96 \\ \cline{2-4}
				& \textbf{TAP-Net++} & \textbf{0.934} & \textbf{9.11} \\ \hline
				\multirow{3}{*}{1} & Greedy EMS & 0.818 & 8.34 \\ \cline{2-4}
				& TAP-Net & 0.553 & 3.75 \\ \cline{2-4}
				& \textbf{TAP-Net++} & \textbf{0.941} & \textbf{9.15} \\ \hline	
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_ppsg_real_multi_all.tex <==
\begin{table}[!t]%
	\caption{\jz{Comparison on the performance of the full pipeline obtained using TAP-Net++ and the two baseline methods. Testing under a realistic scene, ask to pack all the PPSG boxes into multiple containers, the box can be packed in each container.}}
	\label{tab:ppsg_real_multi_all}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l||l|l|l|l}
				\hline
				\textbf{Unit length} &  \textbf{Method} & \bm{$C$} & \bm{$N$} & \bm{$\Delta N$}  \\ \hline 
				\multirow{3}{*}{10} & Greedy & 0.615 & 1.83 & 0.83 \\ \cline{2-5}
				& TAP-Net & 0.492 & 2.05 & 1.05 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.785} & \textbf{1.43} & \textbf{0.43} \\ \hline
				\multirow{3}{*}{5} & Greedy & 0.602 & 1.88 & 0.88 \\ \cline{2-5}
				& TAP-Net & 0.488 & 2.08 & 1.07 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.780} & \textbf{1.44} & \textbf{0.44} \\ \hline
				\multirow{3}{*}{1} & Greedy & 0.560 & 2.02 & 1.02 \\ \cline{2-5}
				& TAP-Net & 0.478 & 2.13 & 1.13 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.761} & \textbf{1.49} & \textbf{0.48} \\ \hline	
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_ppsg_real_multi_last.tex <==
\begin{table}[!t]%
	\caption{\jz{Comparison on the performance of the full pipeline obtained using TAP-Net++ and the two baseline methods. Testing under a realistic scene, ask to pack all the PPSG boxes into multiple containers, the box is only allowed to be packed in the last container.}}
	\label{tab:ppsg_real_multi_last}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l||l|l|l|l}
				\hline
				\textbf{Unit length} &  \textbf{Method} & \bm{$C$} & \bm{$N$} & \bm{$\Delta N$}  \\ \hline 
				\multirow{3}{*}{10} & Greedy & 0.583 & 2.02 & 1.01 \\ \cline{2-5}
				& TAP-Net & 0.485 & 2.09 & 1.09 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.779} & \textbf{1.46} & \textbf{0.46} \\ \hline
				\multirow{3}{*}{5} & Greedy & 0.547 & 2.05 & 1.05 \\ \cline{2-5}
				& TAP-Net & 0.485 & 2.09 & 1.09 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.734} & \textbf{1.54} & \textbf{0.55} \\ \hline
				\multirow{3}{*}{1} & Greedy & 0.544 & 2.14 & 1.14 \\ \cline{2-5}
				& TAP-Net & 0.455 & 2.27 & 1.27 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.731} & \textbf{1.54} & \textbf{0.54} \\ \hline	
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_ppsg_real_single.tex <==
\begin{table}[!t]%
	\caption{\jz{Comparison on the performance of the full pipeline obtained using TAP-Net++ and the two baseline methods. Try to pack the PPSG boxes into one container, the algorithms can only pick up the box along its z-axis}}
	\label{tab:ppsg_real_single}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l||l|l}
				\hline
				\textbf{Unit length} &  \textbf{Method} & \bm{$C$}   \\ \hline 
				\multirow{3}{*}{10} & Greedy & 0.808  \\ \cline{2-3}
				& TAP-Net & 0.594  \\ \cline{2-3}
				& \textbf{TAP-Net++} & \textbf{0.931}  \\ \hline
				\multirow{3}{*}{5} & Greedy & 0.782  \\ \cline{2-3}
				& TAP-Net & 0.596  \\ \cline{2-3}
				& \textbf{TAP-Net++} & \textbf{0.930} \\ \hline
				\multirow{3}{*}{1} & Greedy & 0.764  \\ \cline{2-3}
				& TAP-Net & 0.564  \\ \cline{2-3}
				& \textbf{TAP-Net++} & \textbf{0.929}  \\ \hline	
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_ppsg_real_single_xyz.tex <==
\begin{table}[!t]%
	\caption{\jz{Comparison on the performance of the full pipeline obtained using TAP-Net++ and the two baseline methods. Try to pack the PPSG boxes into one container, the algorithms can pick up the box along its x-axis, y-axis and z-axis.}}
	\label{tab:ppsg_real_single_xyz}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l||l|l}
				\hline
				\textbf{Unit length} &  \textbf{Method} & \bm{$C$}   \\ \hline 
				\multirow{3}{*}{10} & Greedy & 0.752  \\ \cline{2-3}
				& TAP-Net & 0.515  \\ \cline{2-3}
				& \textbf{TAP-Net++} & \textbf{0.897}  \\ \hline
				\multirow{3}{*}{5} & Greedy & 0.731  \\ \cline{2-3}
				& TAP-Net & 0.506  \\ \cline{2-3}
				& \textbf{TAP-Net++} & \textbf{0.880} \\ \hline
				\multirow{3}{*}{1} & Greedy & 0.709  \\ \cline{2-3}
				& TAP-Net & 0.431  \\ \cline{2-3}
				& \textbf{TAP-Net++} & \textbf{0.880}  \\ \hline	
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_rand_ideal_multi_all.tex <==
\begin{table}[!t]%
	\caption{\jz{Comparison on the performance of the full pipeline obtained using TAP-Net++ and the two baseline methods. Testing under ideal scene, ask to pack all the RAND boxes into multiple containers, the box can be packed in each container.}}
	\label{tab:rand_ideal_multi_all}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l||l|l|l|l}
				\hline
				\textbf{Unit length} &  \textbf{Method} & \bm{$C$} & \bm{$N$} & \bm{$\Delta N$}  \\ \hline 
				\multirow{3}{*}{10} & Greedy EMS & 0.601 & 3.04 & 0.91 \\ \cline{2-5}
				& TAP-Net & 0.516 & 3.61 & 1.45 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.649} & \textbf{2.87} & \textbf{0.71} \\ \hline
				\multirow{3}{*}{5} & Greedy EMS & 0.576 & 3.19 & 1.01 \\ \cline{2-5}
				& TAP-Net & 0.467 & 3.98 & 1.79 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.610} & \textbf{3.02} & \textbf{0.83} \\ \hline
				\multirow{3}{*}{1} & Greedy EMS & 0.558 & 3.31 & 1.13 \\ \cline{2-5}
				& TAP-Net & 0.437 & 4.22 & 2.05 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.582} & \textbf{3.18} & \textbf{1.01} \\ \hline	
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_rand_ideal_multi_last.tex <==
\begin{table}[!t]%
	\caption{\jz{Comparison on the performance of the full pipeline obtained using TAP-Net++ and the two baseline methods. Testing under ideal scene, ask to pack all the RAND boxes into multiple containers, the box is only allowed to be packed in the last container.}}
	\label{tab:rand_ideal_multi_last}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l||l|l|l|l}
				\hline
				\textbf{Unit length} &  \textbf{Method} & \bm{$C$} & \bm{$N$} & \bm{$\Delta N$}  \\ \hline 
				\multirow{3}{*}{10} & Greedy EMS & 0.598 & 3.06 & 0.92 \\ \cline{2-5}
				& TAP-Net & 0.516 & 3.62 & 1.46 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.640} & \textbf{2.90} & \textbf{0.74} \\ \hline
				\multirow{3}{*}{5} & Greedy EMS & 0.567 & 3.25 & 1.06 \\ \cline{2-5}
				& TAP-Net & 0.464 & 4.00 & 1.82 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.610} & \textbf{3.04} & \textbf{0.85} \\ \hline
				\multirow{3}{*}{1} & Greedy EMS & 0.544 & 3.40 & 1.23 \\ \cline{2-5}
				& TAP-Net & 0.436 & 4.26 & 2.11 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.567} & \textbf{3.25} & \textbf{1.07} \\ \hline	
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_rand_ideal_single.tex <==
\begin{table}[!t]%
	\caption{\jz{Comparison on the performance of the full pipeline obtained using TAP-Net++ and the two baseline methods. Testing under ideal scene, try to pack the RAND boxes into one container.}}
	\label{tab:rand_ideal_single}
	\begin{minipage}{\columnwidth}
		\begin{center}
		\begin{tabular}{l||l|l|l}
			\hline
			\textbf{Unit length} &  \textbf{Method} & \bm{$C$} & \bm{$N_{\text{box}}$}  \\ \hline 
			\multirow{3}{*}{10} & Greedy EMS & 0.753 & 7.46 \\ \cline{2-4}
								& TAP-Net & 0.508 & 7.22 \\ \cline{2-4}
								& \textbf{TAP-Net++} & \textbf{0.840} & \textbf{8.55} \\ \hline
			\multirow{3}{*}{5} & Greedy EMS & 0.701 & 7.18 \\ \cline{2-4}
								& TAP-Net & 0.435 & 6.33 \\ \cline{2-4}
								& \textbf{TAP-Net++} & \textbf{0.788} & \textbf{8.27} \\ \hline
			\multirow{3}{*}{1} & Greedy EMS & 0.652 & 6.76 \\ \cline{2-4}
								& TAP-Net & 0.407 & 5.78 \\ \cline{2-4}
								& \textbf{TAP-Net++} & \textbf{0.717} & \textbf{7.56} \\ \hline	
		\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_rand_real_multi_all.tex <==
\begin{table}[!t]%
	\caption{\jz{Comparison on the performance of the full pipeline obtained using TAP-Net++ and the two baseline methods. Testing under ideal scene, ask to pack all the RAND boxes into multiple containers, the box can be packed in each container.}}
	\label{tab:rand_real_multi_all}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l||l|l|l|l}
				\hline
				\textbf{Unit length} &  \textbf{Method} & \bm{$C$} & \bm{$N$} & \bm{$\Delta N$}  \\ \hline 
				\multirow{3}{*}{10} & Greedy & 0.503 & 3.74 & 1.60 \\ \cline{2-5}
				& TAP-Net & 0.537 & 3.44 & 1.31 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.622} & \textbf{3.00} & \textbf{0.84} \\ \hline
				\multirow{3}{*}{5} & Greedy & 0.491 & 3.83 & 1.65 \\ \cline{2-5}
				& TAP-Net & 0.454 & 4.10 & 1.92 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.588} & \textbf{3.15} & \textbf{0.97} \\ \hline
				\multirow{3}{*}{1} & Greedy & 0.464 & 4.05 & 1.88 \\ \cline{2-5}
				& TAP-Net & 0.427 & 4.36 & 2.18 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.538} & \textbf{3.49} & \textbf{1.32} \\ \hline	
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_rand_real_multi_last.tex <==
\begin{table}[!t]%
	\caption{\jz{Comparison on the performance of the full pipeline obtained using TAP-Net++ and the two baseline methods. Testing under a realistic scene, ask to pack all the RAND boxes into multiple containers, the box is only allowed to be packed in the last container.}}
	\label{tab:rand_real_multi_last}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l||l|l|l|l}
				\hline
				\textbf{Unit length} &  \textbf{Method} & \bm{$C$} & \bm{$N$} & \bm{$\Delta N$}  \\ \hline 
				\multirow{3}{*}{10} & Greedy & 0.409 & 4.82 & 2.68 \\ \cline{2-5}
				& TAP-Net & 0.457 & 4.05 & 1.92 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.625} & \textbf{2.95} & \textbf{0.81} \\ \hline
				\multirow{3}{*}{5} & Greedy & 0.385 & 5.01 & 2.83 \\ \cline{2-5}
				& TAP-Net & 0.450 & 4.13 & 1.95 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.584} & \textbf{3.19} & \textbf{1.00} \\ \hline
				\multirow{3}{*}{1} & Greedy & 0.377 & 5.14 & 2.97 \\ \cline{2-5}
				& TAP-Net & 0.413 & 4.52 & 2.35 \\ \cline{2-5}
				& \textbf{TAP-Net++} & \textbf{0.522} & \textbf{3.58} & \textbf{1.40} \\ \hline	
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_rand_real_single.tex <==
\begin{table}[!t]%
	\caption{\jz{Comparison on the performance of the full pipeline obtained using TAP-Net++ and the two baseline methods. Try to pack the RAND boxes into one container.}}
	\label{tab:rand_real_single}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l||l | l}
				\hline
								
				\textbf{Unit length} &  \textbf{Method} & \bm{$C$}  \\ \hline 
				\multirow{3}{*}{10} & Greedy & 0.585  \\ \cline{2-3}
									& TAP-Net & 0.485  \\ \cline{2-3}
									& \textbf{TAP-Net++} & \textbf{0.816} \\ \hline
				\multirow{3}{*}{5} & Greedy & 0.533 \\ \cline{2-3}
									& TAP-Net & 0.404  \\ \cline{2-3}
									& \textbf{TAP-Net++} & \textbf{0.742} \\ \hline
				\multirow{3}{*}{1} & Greedy & 0.514 \\ \cline{2-3}
									& TAP-Net & 0.345  \\ \cline{2-3}
									& \textbf{TAP-Net++} & \textbf{0.656} \\ \hline	
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_scalability_num.tex <==
\begin{table}[!t]%
	\caption{\jz{Scalability on box num $N_s$. }}
	\label{tab:tab_scalability_num}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l||l | l | l }
				\hline
				
				\textbf{\bm{{$N_s$}}} &  \bm{$C$} & \bm{$N$} & \bm{$\Delta N$}   \\ \hline 
				20 & 0.540  &  3.46  & 1.28   \\ \hline
				40 & 0.583  & 6.30   & 2.21   \\ \hline
				60 & 0.586  &  9.39  &  3.42  \\ \hline
				80 & 0.582  &  12.60  &  4.79  \\ \hline
				100 &  0.575 &  15.96  &  6.32  \\ \hline
				
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/tab_scalability_pratical.tex <==
\begin{table}[!t]%
	\caption{\jz{Generality on practical settings.}}
	\label{tab:tab_generality_practical}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l||l | l | l }
				\hline
				
				  &  \bm{$C$} & \bm{$N$} & \bm{$\Delta N$}   \\ \hline 
				Greedy &   &    &    \\ \hline
				TAP-Net &   &    &    \\ \hline
				TAP-Net++ &   &    &    \\ \hline
				
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%

